Demystifying the Characteristics of 3D-Stacked Memories: A Case Study for Hybrid Memory Cube

Three-dimensional (3D)-stacking technology, which enables the integration of DRAM and logic dies, offers high bandwidth and low energy consumption. This technology also empowers new memory designs for executing tasks not traditionally associated with memories. A practical 3D-stacked memory is Hybrid Memory Cube (HMC), which provides significant access bandwidth and low power consumption in a small area. Although several studies have taken advantage of the novel architecture of HMC, its characteristics in terms of latency and bandwidth or their correlation with temperature and power consumption have not been fully explored. This paper is the first, to the best of our knowledge, to characterize the thermal behavior of HMC in a real environment using the AC-510 accelerator and to identify temperature as a new limitation for this state-of-the-art design space. Moreover, besides bandwidth studies, we deconstruct factors that contribute to latency and reveal their sources for high- and low-load accesses. The results of this paper demonstrates essential behaviors and performance bottlenecks for future explorations of packet-switched and 3D-stacked memories.

==> tex/ad.tex <==
%Submission and reviewing guidelines and methodology: \\
%{\small\em http://sc17.supercomputing.org/submitters/technical-papers/reproducibility-initiatives-for-technical-papers/artifact-description-paper-title/}
\label{sec:AD}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}
To obtain the GUPS infrastructure, this artifact contains the code that  
enables applying the modifications for repeating the experiments in this paper. 
%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}
As mentioned in Section~\ref{sec:meth-firm}, we use three implementations of GUPS:
(1) Full-scale, (2) Small-scale, and (3) Stream GUPS. 
%
While two former ones contain some minor modifications of the base code, 
obtainable from PicoComputing
~\cite{hmc-framework}, the latter one includes major modifications.
%
%The base version of the first two is obtainable from PicoComputing
%~\cite{hmc-framework} plus
%some minor modifications, while the latter also contains major modifications.
%
In this artifact, we provide our scripts and describe the modifications.


%---------------------------------------------------%
\subsubsection{Check-List}

{\small
\begin{itemize}
  \item {\bf Algorithm: Giga updates per second (GUPS), and a custom request generator based on Xilinx's AXI-Stream interface.}
  \item {\bf Program: Verilog, and C++.}
  \item {\bf Compilation: g++ 4.8.4, and Xilinx Vivado 2016.1.}
  \item {\bf Binary: See Section~\ref{sec:ad-install}.}
  \item {\bf Data set: See Section~\ref{sec:ad-dataset}.}
  \item {\bf Run-time environment: Ubuntu 14.04.2 LTS.}
  \item {\bf Hardware: an AC-510 accelerator board~\cite{ac510}, an EX-700 PCIe backplane~\cite{ex700}, a thermal camera,  and a power analyzer.}
  \item {\bf Run-time state: The system, HMC, and FPGA are idle and only running experiments. Room temperature of $25$\textdegree C.}
  \item {\bf Execution: 20 seconds for bandwidth and 200 seconds for thermal and power experiments. See Section~\ref{sec:ad-workflow}.}
  \item {\bf Output: GUPS stats, thermal and power numbers.}
  \item {\bf Experiment workflow: See Section~\ref{sec:ad-workflow}.}
  \item {\bf Publicly available?: Yes.}
\end{itemize}
}


%---------------------------------------------------%
\subsubsection{How Software Can be Obtained}
To obtain Pico API\-~\cite{pico-api}, HMC Controller~\cite{hmc-controller}, 
and GUPS digital design 
(\texttt{HMC\_release\-\_4.0} and \texttt{picocomputing-5.4.2.0/}), 
please email \href{mailto:hpc@micron.com}{hpc@micron.com}\-~\cite{hmc-framework}.
%
The rest of scripts are described in the following sections.


%---------------------------------------------------%
\subsubsection{Hardware Dependencies}
Experiments are performed on an HMC prototype on AC-510 accelerator board~\cite{ac510} that is
on an EX-700 PCIe backplane~\cite{ex700}, obtainable from PicoComputing.
%
As Section~\ref{sec:meth-inf} describes, we use a thermal camera~\cite{flir-camera} 
for thermal measurements, and a power analyzer~\cite{extech}
for power measurements of the machine.

%---------------------------------------------------%
\subsubsection{Software Dependencies}
We execute the experiments on Ubuntu 14.04.2 LTS with g++ 4.8.4, but no strict
dependencies exist. 
%
For digital design compilations we 
use Xilinx Vivado Design Suite version 2016.1.

%---------------------------------------------------%
\subsubsection{Datasets}
\label{sec:ad-dataset}
Based on the given parameters to GUPS, access patterns to HMC are generated 
within the FPGA.
We provide extra details in Section~\ref{sec:ad-workflow} .

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation and Modifications}
\label{sec:ad-install}
The Pico framework on the system is required.
%
To do so, after obtaining \texttt{picocomputing-5.4.2.0/} or a newer version, do:
\begin{lstlisting}[numbers=left]
sudo dpkg -i picocomputing_5.4.2.0_all.deb
\end{lstlisting}
%
Afterwards, based on the experiments, we load the FPGA with the appropriate digital design.
%---------------------------------------------------%
\subsubsection{Full-Scale and Small-Scale GUPS}
To program the FPGA, for full-scale and small-scale GUPS implementation, we use the provided bitfile
in \texttt{HMC\_release\_4.0}. After execution of \texttt{make} in \texttt{GUPS/software}, do:
\begin{lstlisting}[numbers=left]
./gups loadall --b ../firmware/M510_KU060_GUPS.bit
\end{lstlisting}
%
Between the experiments, we program the FPGA to reset the stat counters.
%
In addition, in the provided software for GUPS, we add input command line parameters of
\texttt{mask} and \texttt{anti-mask}.
%
Also, we modify statistics function of GUPS to print latency related statistics.

%---------------------------------------------------%
\subsubsection{Stream GUPS}
\label{sec:stream-gups}
Stream GUPS uses a customized GUPS that utilizes Xilinx's AXI-Stream interface to send/receive 
commands/responses from the FPGA with a high speed. Here, we present an overview of our modifications.
%
Each GUPS module has two bi-directional streams that are used to (1) receive 
read/write commands from the host and (2) send the read response back to the host. 
%
The top level module is connected to two read and two write streams. 
%
Each stream 
port has a valid and ready signal that is used for handshaking and a data port 
contains 128-bit data during each cycle of the stream clock (250\,MHz).
%
The command input stream is connected to a command buffer which is in turn 
connected to the read request FIFO 
and a write request FIFO. 
%
Each command is 128 bits, with bits 33-0 containing the address, 
bit 34 designating either a read or a write, and bits 35-38 containing the size of the request.
% 
Read requests are fetched by the read request FIFO and 
write requests are fed into the write request FIFO. 
%
The write data stream is connected to a write data FIFO, which contains 
data required to be written to the HMC corresponding 
to a write request in the command FIFO.
%
The read request FIFO module handles read requests and their corresponding read responses. 
The address and size outputs are connected to a read address FIFO that is in turn connected 
with the address output stream data allowing us to identify the membership of the read data 
that is returned from the HMC.
%
In a similar way, data read from the HMC is also fed into a read data FIFO which in 
turn is connected to the read data output stream.
%
After above modification to the digital design, we compiled and load it to the
FPGA in a similar way to full-scale and small-scale GUPS.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Workflow of Experiments}
\label{sec:ad-workflow}
This section describes experiment workflows and provide the scripts.
%
Each script prints out the results on CLI. To save space, we do not include 
commands related to parsing the results.
%
For running each experiment, we set required registers in the FPGA. 
%
While the experiments are running on the FPGA, we read the stats in the period
of 20 or 200 seconds. 
%
Note that reading the statistics does not affect FPGA execution or timings.
Therefore, the host does not intervene in the process of monitoring the stats or make the stats
inaccurate by reading them.

%---------------------------------------------------%
\subsubsection{Address Mapping Experiments}
For address mapping experiments we shifted eight-bit mask operation on random addresses, 
here is the python code we use to run this experiment.
%
\begin{lstlisting}[language=Python, showstringspaces=false]
for i in range(0,25):
  tmpMask=bit_not(0xFF000000 >> i)
  masks8.append(tmpMask)
for i in range(len(masks8)):
  os.system('./gups gups_std --m 0x510 --size 8 --ports 9 --ro --mask %#x --anti_mask 0x00'  % ( masks8[i]))
\end{lstlisting}
%
\texttt{--size} specifies the size of request in 16B granularities. \texttt{--ports} specifies the number
of active GUPS ports. \texttt{--ro} specifies type of request (read only in this case).

%---------------------------------------------------%
\subsubsection{Bandwidth, Thermal, and Power Experiments}
For bandwidth, thermal, and power experiments we use the code in below. However, in the software, we use
\texttt{usleep()} function to lengthen the execution time for thermal and power experiments from 20
to 200 seconds.
%
By changing \texttt{anti\_mask} we target vaults, banks, and quadrants. 
The final reported results is an average across all possible combinations.
%
\begin{lstlisting}[language=bash, keepspaces=true]
for SIZE in $(seq 1 8)
do
  for TYPE in "ro" "wo" "rw"
  do
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --${TYPE}   --mask 0xffffffff  --anti_mask 0x00000000
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --${TYPE}   --mask 0xfffffbff  --anti_mask 0x00000000
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --${TYPE}   --mask 0xfffff9ff  --anti_mask 0x00000000
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --${TYPE}   --mask 0xfffff97f  --anti_mask 0x00000000
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --${TYPE}   --mask 0xfffff87f  --anti_mask 0x00000000
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --${TYPE}   --mask 0xffffb87f  --anti_mask 0x00000000
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --${TYPE}   --mask 0xffff987f  --anti_mask 0x00000000
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --${TYPE}   --mask 0xffff887f  --anti_mask 0x00000000 
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --${TYPE}   --mask 0xffff807f  --anti_mask 0x00000000
  done
done
\end{lstlisting}
%
We performed the experiments several time, and reported the average values in the paper.

%---------------------------------------------------%
\subsubsection{Close-page Policy Experiments}
For close-page policy experiments, we use linear and random mode of addressing. 
The code in below produces the same result shown in Figure~\ref{fig:res-bw-open}.
However, to see if the trend is the same, we execute all possible combinations and patterns.

\begin{lstlisting}[language=bash, keepspaces=true]
for SIZE in $(seq 1 8)
do
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --ro                --mask 0xffffffff  --anti_mask 0x00000000
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --ro                --mask 0xfffff87f  --anti_mask 0x00000000
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --ro  --linear     --linear-step ${SIZE} --mask 0xffffffff  --anti_mask       0x00000000
  ./gups gups_std --m 0x510 --size ${SIZE} --p 9 --ro  --linear     --linear-step ${SIZE} --mask 0xfffff87f  --anti_mask       0x00000000
done

\end{lstlisting}

%---------------------------------------------------%
\subsubsection{Low-Load Access Latency Experiments}
For low-load access latency we use the stream GUPS implementation. As mentioned in 
Section~\ref{sec:stream-gups}, for read accesses, we created one stream that contains
the addresses, size, and the command for read requests.
%
Here is the code snippet of how we fill the command stream.  
%
\begin{lstlisting}[language=C++]
for(i=0; i<words*4; i+=4)
{
  //-serial accesses
  //buf[j] = start_address + (i/4*size_each_word);
  //--stressing just one bank in one vault
  //buf[i] = start_address + (i/4*0x8000);
  //--spreading out across vaults
  buf[i] = start_address + (i/4*0x80);
  buf[i+1] = ((size_each_word/16) << 3) | (0 << 2);
  buf[i+2] = 0;
  buf[i+3] = 0;
}
\end{lstlisting}
%
The results presented for low-load access latency are when we spread out the
accesses across vaults.
%
To change the number of requests, the port number from which we issue request to HMC, and
size of each request, we change the software to accept command line parameters.
%
Then, we run the experiments with the code below, and take the average of all the results.
%
\begin{lstlisting}[keepspaces=true]
./gups loadall --b Pico_Toplevel_streamGUPS.bit
./gups gups_setup --m 0x510 --p 9
SIZE=128
for WORDS in $(seq 1 30)
do
  for STREAM in $(seq 1 2 17) # each port has two streams to HMC, 
                              # one commands, one data (writes)
  do
    ./gups gups_test_read_write --m 0x510 --stream_module $STREAM   --stream_address 0x46300000 --stream_number_of_words $WORDS --stream_size_word $SIZE
  done
done
\end{lstlisting} 

%---------------------------------------------------%
\subsubsection{Bandwidth-Latency Relationship Experiments}
For measuring bandwidth-latency relationship, we use small-scale GUPS. 
%
\begin{lstlisting}[language=bash, keepspaces=true]
for SIZE in $(seq 1 8) #16B chunks
for PORT in $(seq 1 9) #from one port to all port active
do
  for TYPE in "ro" "wo" "rw"
  do
    ./gups loadall --b ./Pico_Toplevel_smallGUPS.bit
    ./gups_mask gups_std --m 0x510 --size ${SIZE} --p ${PORT}       --${TYPE} --mask 0xffffffff --anti_mask 0x00000000
    ./gups_mask gups_std --m 0x510 --size ${SIZE} --p ${PORT}       --${TYPE} --mask 0xfffffbff --anti_mask 0x00000000
    ./gups_mask gups_std --m 0x510 --size ${SIZE} --p ${PORT}       --${TYPE} --mask 0xfffff9ff --anti_mask 0x00000000
    ./gups_mask gups_std --m 0x510 --size ${SIZE} --p ${PORT}       --${TYPE} --mask 0xfffff97f --anti_mask 0x00000000 
    ./gups_mask gups_std --m 0x510 --size ${SIZE} --p ${PORT}       --${TYPE} --mask 0xfffff87f --anti_mask 0x00000000
    ./gups_mask gups_std --m 0x510 --size ${SIZE} --p ${PORT}       --${TYPE} --mask 0xffffb87f --anti_mask 0x00000000
    ./gups_mask gups_std --m 0x510 --size ${SIZE} --p ${PORT}       --${TYPE} --mask 0xffff987f --anti_mask 0x00000000
    ./gups_mask gups_std --m 0x510 --size ${SIZE} --p ${PORT}       --${TYPE} --mask 0xffff887f --anti_mask 0x00000000
    ./gups_mask gups_std --m 0x510 --size ${SIZE} --p ${PORT}       --${TYPE} --mask 0xffff807f --anti_mask 0x00000000
    ./gups_mask gups_stop --m 0x510
  done
done
\end{lstlisting}
%
As the code snippets shows, we run several experiments for all types of requests and sizes.
%
In the paper, we have shown read-only requests, and a few of sizes. However, we verified the
trend is similar to what is shown in Figure~\ref{fig:res-latency}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tex/cra.tex <==
%Submission guidelines: \\
%{\small\em http://sc17.supercomputing.org/submitters/technical-papers/reproducibility-initiatives-for-technical-papers/computational-results-analysis-paper-title/}
\label{sec:CRA}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}
Since this paper focuses on performance and thermal measurements for a device
with limited availability, in this section we provide an overall description of
how we ensure the quality and trustworthiness of our results. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Results Analysis Discussion}


\subsubsection{The Integrity of Communication Layers}
\label{sec:CRA-integrity}
%
In this paper we evaluate various aspects of a system that contains 
an HMC evaluation board.
%
For such a system that several hardware components communicate with a host and 
its software, many layers of software/hardware are implemented.
%
In our system, the host communicates with the FPGA on the AC-510 board~\cite{ac510}, and
then FPGA sends requests and receive responses from the HMC.
%
Therefore, the first layer is the communication between the host and the FPGA.
%
To command the FPGA to perform a task, the host sets the value of control 
registers inside the FPGA via Pico API~\cite{pico-api}.
%
This mode of command is for full-scale and small-scale GUPS (see Section~\ref{sec:meth-inf}).
%
We verify that a value is propagated from the host to the FPGA by reading the values of the registers.
%
Besides the configuration, the statistics (e.g., number of accesses, read latency, and etc.) are also transmitted in this fashion (i.e., via some registers).
%
The second layer of communication is between the FPGA and the HMC. In the FPGA, various 
statistics registers are implemented for monitoring the issuance/reception 
of requests/responses. 
%
To ensure that a memory transaction was successful, the FPGA checks the written value afterwards.
%However, the only way of ensuring that a memory transaction was successful 
%is by checking its value afterwards. 
%
For instance, if we write X to location A, a read of location A should return X.
%
Ultimately, in communication between the FPGA and HMC, the FPGA ensure the correctness  of transactions in two ways:
(1) The stream GUPS uses the read-after-write method to ensure data integrity.
%
(2) Counters implemented on the FPGA check failed transactions by matching number of received acknowledgements against number of all transactions.
%
%The counter of failed transactions on the FPGA. by 
%using the counter we ensure that the FPGA received an acknowledgement for all transactions
(This acknowledgment is for the physical layer of the AXI transfer protocol).
%
 



\subsubsection{Timing Measurements for Bandwidth Calculations}
To calculate bandwidth in this paper, we use the statistic registers in the FPGA,
and a host timer.
%
The statistics report the number of accesses executed during an elapsed time. 
%
We calculate number of transferred byte by multiplying number of request and response  
packets to their corresponding size including data payload and overhead, based on Table~\ref{tab:hmc-rdwrsize}. 
%To get the number of bytes transferred (payload and overhead), we use the numbers in 
%Table~\ref{tab:hmc-rdwrsize}.
%
To verify the number of calculated bytes, we compared them with number of transferred bytes that is 
also monitored separately by FPGA and is sent to the host in a statistic register.
%
%We verify the calculated payload values with the reported values from the FPGA, 
%that is number of bytes accessed for reads or writes.
%
To measure the duration of time, in which a particular number of bytes are transferred, 
we use a timer in the host.
%the following technique.
%
All in all, the steps of calculating bandwidth are the following:
First, the GUPS module starts accessing the HMC iteratively, based on its dedicated configuration.
Then, right before starting the timer, we read the statistics registers for initial values of number of reads/writes. 
After that, we start the timer and wait for 20 or 200 seconds based on the type of the experiment. 
%
Finally, we read the statistics registers again for the final values of number of reads/writes, 
and subtract the initial values from them, and divide the number of bytes 
(calculated and verified as mentioned above) by the elapsed time.
%
As mentioned steps do not intervene with the process on the FPGA, and as the process of reading
registers takes little time (comparing to overall elapsed time), the reported values for bandwidth are precise.


\subsubsection{Thermal and Power Measurements}
As discussed in Section~\ref{sec:res-th-pow}, our
thermal measurements are limited by the resolution of our infrastructure, so the absolute 
temperature values are an approximation.
%
However, the important fact is the relative trend of temperature and power consumption 
for access patterns.
%
We ensured the trends are correct by repeating the experiments. In all repeated experiments 
we see the same trend in temperature.

\subsubsection{Performance Results}
\label{sec:CRA-perf}

In the paper, reported results for bandwidth and latency of access patterns 
are verified by repeating them. We report the average value across all experiments. 
%
As discussed and presented in appendix~\ref{sec:AD}, we can execute most of the
experiments in various ways. For instance, to target a bank within a vault, we have
multiple options to choose the bank number. For these type of experiments, 
we tried sufficient permutations, so we observe any discrepancy. However,
the observed results followed the same trend and approximately same values.
%
Therefore, we reported the average value.
%
In addition, as mentioned in Section~\ref{sec:CRA-integrity}, FPGA counters enabled
us to verify correct execution of each experiment and its results.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Summary}
%
In summery, we ensured the quality and trustworthiness of our results by repeating the
experiments, monitoring the statistic counters, and reporting the average of multiple 
permutations for each experiment.



